"A Special Operation": A Quantitative Approach to Dissecting and Comparing Different Media Ecosystems' Coverage of the Russo-Ukrainian War

The coverage of the Russian invasion of Ukraine has varied widely between Western, Russian, and Chinese media ecosystems with propaganda, disinformation, and narrative spins present in all three. By utilizing the normalized pointwise mutual information metric, differential sentiment analysis, word2vec models, and partially labeled Dirichlet allocation, we present a quantitative analysis of the differences in coverage amongst these three news ecosystems. We find that while the Western press outlets have focused on the military and humanitarian aspects of the war, Russian media have focused on the purported justifications for the "special military operation" such as the presence in Ukraine of "bio-weapons" and "neo-nazis", and Chinese news media have concentrated on the conflict's diplomatic and economic consequences. Detecting the presence of several Russian disinformation narratives in the articles of several Chinese outlets, we finally measure the degree to which Russian media has influenced Chinese coverage across Chinese outlets' news articles, Weibo accounts, and Twitter accounts. Our analysis indicates that since the Russian invasion of Ukraine, Chinese state media outlets have increasingly cited Russian outlets as news sources and spread Russian disinformation narratives.

==> background.tex <==
\section{Background}

==> canned.tex <==
\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{\multirow{2}{*}{Topic}}  & \multicolumn{2}{c|}{Western}  & \multicolumn{2}{c|}{Russian} & \multicolumn{2}{c|}{Chinese}\\ \cline{2-7}
   &{Keywords} & {\# Art.} & {Keywords}  & {\# Art.}   & {Keywords}  & {\# Art.}            \\   \hline 
  Topic 1  & russian,force,ukrainian,city,kyiv,ukraine,russia,troop,military & 411 & kiev,russian,ukraine,ukrainian,military,operation,donbass   &  302  & china wang ukraine taiwan issue &  220           \\ \hline
 Topic 2  & family,day,war,russian,people,ukrainian,kyiv & 250 & russian,force,ukrainian,military,armed,city,dpr   &   275   &ukraine security, china, un, crisis, peace& 214             \\ \hline
  Topic 3  & ukraine,news,president,biden,zelenskyy,putin & 182   & ukrainian,bucha,russian,nazi,video,azov,civilian   &  143  & ukraine, talk, russia, roud, delegation & 202           \\ \hline
 Topic 4& ukraine,zelensky,russia,report,trust &151 & kiev,ukrainian,nazi,operation,foreign,german   & 84  & percent price ukraine global conflict food & 133 \\   \hline
  Topic 5  & war,crime,civilian,bucha,russian,body,kill,genocide & 149  & us,ukraine,biological,weapon,russian,military  &  83   &biological us  ukraine weapon  weapon  laboratory & 89          \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}



\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 1}  &{Week 2} &{Week 3} &{Week 4}\\\hline
  Western Press  &  troops ukrainian forces military russian-backed &kyiv ukrainian troops crimea units & trump electors state campaign michigan & breyer court photos justice supreme
          \\ \hline
 Russia & russian,ukrainian,vessel,yanukovych,inland &russia russian nato intelligence ukrainian& kiev, erdo, eu, claim, medium&   russia russian kiev ukrainian athletes 
        \\ \hline
  Chinese  &cooperation china bilateral development diplomatic  &  nuclear,china,ukraine,country,russia & say, china, pipeline, germany, europe  &  russia russian nato kiev united  \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}


\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 5}  &{Week 6} &{Week 7} &{Week 8}\\\hline
  Western Press &  kyiv belarus putin eastern people & sunday diplomatic scholz house macron military moscow kiev president media &intelligence official attack belarus sullivan &officials pretext zelenskiy reports russians
          \\ \hline
 Russia  &russia russian ukrainian kiev turkish& military moscow kiev president media & military nato moscow president country & nato invasion moscow president security
        \\ \hline
  Chinese  &china security council tensions parties  & russia military joint deploy statement &moscow putin ukrainian nato security &president,ukrainian,security,putin,military,nato\\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}

\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 9}  &{Week 10} &{Week 11} &{Week 12}\\\hline
  Western Press &  world support speech news photos & news zelenskyy ukrainians told kharkiv& mage know speaking sabrina tavernise  &  zelenskyy putin kyiv news forces
          \\ \hline
 Russia  & forces putin donbass country republics &kiev operation people putin special &  people operation kiev president putin &  kiev president operation people donbass

        \\ \hline
  Chinese &china putin military president ukrainian& russian,china,military,security,chinese  &china chpresident,military,countries,crisis & china russian ukrainian president military \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}

\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 9}  &{Week 10} &{Week 11} &{Week 12}\\\hline
  Western Press &  kyiv,city,forces,killed,troops,shelling &city,mariupol,kyiv,lviv,monday,shelling &town,civilians,killed,officials,zelenskiy &military,kyiv,invasion,putin,forces,zelenskyy
          \\ \hline
 Russia  & donbass,republics,biological,defense,laboratories&kiev,forces,country,president,special,operation & kiev,forces,people,operation,president,donbass,special &kiev,president,republics,operation,donbass, lugansk

        \\ \hline
  Chinese &  crisis,countries,conflict,international,chinese&china,military,president,people,country,forces,foreign & military,security,president,people,peace,chinese,crisis & peace,ukrainian,foreign,world,president,international,cold\\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}


\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{\multirow{2}{*}{Topic}}  & \multicolumn{2}{c|}{Western}  & \multicolumn{2}{c|}{Russian} & \multicolumn{2}{c|}{Chinese}\\ \cline{2-7}
   &{Keywords} & {\# Art.} & {Keywords}  & {\# Art.}   & {Keywords}  & {\# Art.}            \\   \hline 
  Topic 1  & city,mariupol,kyiv,forces,zelenskiy,region,civilians & 511 & president,putin,operation,kiev,people,special,country,donbass,  &  302  & china,security,wang,chinese,crisis,peace,situation &  475           \\ \hline
 Topic 2  & family,want,kyiv,time,news,home & 336 & forces,armed,city,units,defense,people,mariupol,region,destroyed  &   320   &china,chinese,wang,taiwan,two,people& 215             \\ \hline
  Topic 3  & forces,kyiv,troops,soldiers,russians,ukrainians,fighting & 270   & kiev,country,moscow,biological,president,minsk,republics,donbass  &  257  & china,military,crisis,conflict,countries,taiwan & 160           \\ \hline
 Topic 4& zelenskyy,news,children,world,killed,says,city,share,civilians &186 & bucha,kiev,people,civilians,azov,crimes &245  & biological,chinese,ministry,weapons,zhao,laboratories & 141 \\   \hline
  Topic 5  & bucha,crimes,civilians,image,bodies,genocide,atrocities& 173  &foreign,president,training,turkey,mercenaries,country,  &  76   &percent,growth,economic,conflict,economy,inflation & 137          \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}


\begin{table}
\centering
\tiny
\begin{tabular}{r|r|r|r|r|r}
\hline  \multicolumn{2}{c|}{Western}  & \multicolumn{2}{c|}{Russian} & \multicolumn{2}{c|}{Chinese}\\ \hline
   {Keyword} & {F-score} & {Keyword}  & {F-score.}   & {Keyword}  & {F-score}            \\\hline 
  zelenskiy  & 1.0 &   dpr &  0.996380    &   zhang   & 1.000000 \\ \hline 
  mile  & 0.988870 &    lpr &  0.995192  &    wang  & 0.999943
  \\ \hline 
  listen  & 0.986305 &   donbass &  0.994088  &  china     & 0.996572 \\ \hline 
  zelenskyy  & 0.978164 &   lugansk & 0.993878  &    growth  & 0.995726
    \\ \hline 
  invasion  & 0.974998 &    kiev & 0.991826      &   percent   &0.994792	 \\ \hline 
  separatist  & 0.974439 &  afu &   0.989532    & stability  & 0.994672
  \\ \hline 
  kyiv  & 0.973661 &     neo-nazi & 0.986864    &  dialogue    & 0.993380  \\ \hline 
  lviv  & 0.967852 &    nationalist &  0.981189     & zhao   &  0.992539  \\ \hline 
  ukrainians  &0.964600 &   coup &  0.979579     &   promote  &  0.991933 \\ \hline 
  kharkiv  & 0.964170 &     provocation & 0.971242     &  taiwan &  0.989373  \\ \hline 
\end{tabular}
\caption{\label{tab:precision}Most characteristic words for each ecosystem across all news articles . }  
\vspace{-10pt}
\end{table}

 \begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/western_vs_russia.png}
\caption{Comparison of the word frequencies between the Western Press and Russian disinformation media. }
\label{fig:western-russian}
\vspace{-10pt}
\end{figure}

 \begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/western_vs_chinese.png}
\caption{Comparison of the word frequencies between the Western Press and Chinese state media. }
\label{fig:western-chinese}
\vspace{-10pt}
\end{figure}

 \begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/russian_vs_chinese.png}
\caption{Comparison of the word frequencies between the Russian disinformation and Chinese State media. }
\label{fig:western-russian}
\vspace{-10pt}
\end{figure}

\begin{table}
\centering
\tiny
\begin{tabular}{r|r|r|r}
\hline  \multicolumn{2}{c|}{Russian}  & \multicolumn{2}{c|}{China} \\ \hline
   {Keyword} & {F-score} & {Keyword}  & {F-score.}         \\\hline 
  neo-nazi  & 1.0 &   zhang &  1.000000    \\ \hline 
  nationalist  & 0.990160&    wang & 0.999793
 
  \\ \hline 
  dpr  & 0.990149 &   percent &0.997118\\ \hline 
  defence  &0.988330 &   china &0.992312
 
    \\ \hline 
  regime  & 0.984920&    growth &0.988784
     	 \\ \hline 
  azov  & 0.984677 &  stability &  0.988557		 
  \\ \hline 
  donbass  & 0.984567 &     taiwan &0.988106
    \\ \hline 
  battalion  &0.984206 &   xi & 0.987672	
   \\ \hline 
  lpr  &0.982216 &   food & 0.984240 \\ \hline 
  lugansk  &0.978011 &     dialogue & 0.984017	
      \\ \hline 
\end{tabular}
\caption{\label{tab:precision}Most characteristic words comparing the Russian and Chinese newspaper ecoystems.  }  
\vspace{-10pt}
\end{table}


\begin{table}
\centering
\tiny
\begin{tabular}{r|r|r|r}
\hline  \multicolumn{2}{c|}{Western}  & \multicolumn{2}{c|}{Chinese} \\ \hline
   {Keyword} & {F-score} & {Keyword}  & {F-score.}         \\\hline 
  zelenskiy  & 1.0 &   wang &  1.000000    \\ \hline 
  mile  & 0.992304&    zhang & 0.999806
 
  \\ \hline 
  listen  & 0.987096 &   kiev & 0.999484 \\ \hline 
  russians  & 0.985966 &   china & 0.995715
 
    \\ \hline 
  invasion  & 0.985798&    dialogue & 0.994210
     	 \\ \hline 
  defence  & 0.980849 &  growth &  0.993269	 
  \\ \hline 
  ukrainians  & 0.980123 &     cooperation &0.993107
    \\ \hline 
  assault  &0.978543 &   promote & 0.992690
   \\ \hline 
  crime  &0.977103 &   stability & 0.992276  \\ \hline 
  resistance  &0.975352 &     li & 0.990747	
      \\ \hline 
\end{tabular}
\caption{\label{tab:precision}Most characteristic words comparing the Western and Chinese newspaper ecoystems.  }  
\vspace{-10pt}
\end{table}


\begin{table}
\centering
\tiny
\begin{tabular}{r|r|r|r}
\hline  \multicolumn{2}{c|}{Western}  & \multicolumn{2}{c|}{Russian} \\ \hline
   {Keyword} & {F-score} & {Keyword}  & {F-score.}         \\\hline 
  zelenskiy  & 1.0 &   kiev &  1.000000    \\ \hline 
  zelenskyy  & 0.995724 &    lpr &  0.999199
 
  \\ \hline 
  kyiv  & 0.992244 &   dpr & 0.998902  \\ \hline 
  mile  & 0.986316 &   lugansk & 0.998845
 
    \\ \hline 
  shelter  & 0.985810 &    donbass & 0.997620
     	 \\ \hline 
  lviv  & 0.985710 &  afu &  0.987364  
  \\ \hline 
  listen  & 0.984848 &     minsk &0.986339
    \\ \hline 
  separatist  &0.981886 &    neo-nazi & 0.984622
   \\ \hline 
  flee  &0.980745 &   nationalist &  0.981182   \\ \hline 
  invasion  & 0.974317 &     stress & 0.979203
      \\ \hline 
\end{tabular}
\caption{\label{tab:precision}Most characteristic words comparing the Russian and Western newspaper ecoystems.  }  
\vspace{-10pt}
\end{table}


\paragraph{Western Press vs Russian Disinformation}
While each media ecosystem largely covers the war in detail as was seen in the previous section, Western Press and Russian disinformation ecosystem have largely different means of  


In addition, we further see prominently, heavy mentions of the eastern Ukrainian region of Donbas, a  separatist area that claimed independence at the beginning of the Russo-Ukrainian War as well as mentions of Ukraine as being filled with Nazis. 
Looking at Table 

\paragraph{Western Press vs Chinese State Media} 
As seen in Figure~\ref{fig:western-chinese}, we again see the distinction that Chinese state media continues to use the Russian spelling of Kyiv. Besides this, we see an emphasis, looking at the characteristic words differentiating Chinese  media from Western press on economic stability and growth. We further see within this dataset, the emphasis on ``cooperation'' and ``dialogue'', which is largely absent from the Western press articles. In contrast, the Western press' main idiosyncratic words have to with the ``crimes, assaults and bodies' in Ukraine. The Western press furthermore were more likely to use words like "invaded."



Besides the the differentiating factor that the Chinese media is more concentrated on economic issues and the Western press on crimes in Ukraine, we further see an emphasis in the Chinese media on biological weapons.




\paragraph{Russian Disinformation vs Chinese State Media} 
Looking at the comparison between Russian and Chinese state media, we again see the characteristic aspects previously discussed for both ecosystems. We see that Chinese state media is largely focused on economic growth and stability; in contrast Russian disinformation largely concerns the previously discussed idea of the Ukraianians being neo-NAZIs as well as particular aspects on different fonts of the ward, especially the Donbas regions. 





\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 1}  &{Week 2} &{Week 3} &{Week 4}\\\hline
  Western Press & kazakhstan crisis kyiv concerns soviet & control crimea american intelligence ground & blinken official geneva meet department & belarus soldiers region attack tanks
          \\ \hline
 Russia &radzikhovsky applebaum putin military invade &  forces,intelligence,according,invasion,kiev,training,nato & nato invasion security president troops &nato moscow president troops forces
        \\ \hline
  Chinese &countries ties cooperation relations zelensky &moscow west cooperation president eastern &nato military president ukrainian talks &  nato russian military ukrainian security \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}



\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 5}  &{Week 6} &{Week 7} &{Week 8}\\\hline
  Western Press &defense video west crimea exercises &sunday diplomatic house sullivan white & house friday sullivan intelligence white &intelligence,official,false,eastern,state,pretext
          \\ \hline
 Russia &nato military kiev invasion moscow &military nato government putin invasion & military president nato putin moscow & invasion moscow nato security president
        \\ \hline
  Chinese & council,countries,states,europe,parties,dialogue&military soldiers poland security deploy & moscow putin macron ukrainian security & president putin security ukrainian military\\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}

\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 9}  &{Week 10} &{Week 11} &{Week 12}\\\hline
  Western Press &thursday attack city ukrainians official & city ukrainians video russians fight
          &  forces kyiv city mariupol civilians & city kyiv forces mariupol killed \\ \hline
 Russia &forces putin donbass republics lugansk & kiev operation president people special & kiev people forces operation ministry  kiev,operation,ministry,president,civilians,donetsk,defense,donbass
        \\ \hline
  Chinese & military,security,people,ukrainian,issue,taiwan &china,russian,security,military,president& russian,ukrainian,foreign,wang,humanitarian & ukrainian,security,russian,crisis,peace,humanitarian\\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}

\begin{table*}
\centering
\tiny
\begin{tabular}{l|r|r|r|r|r|r}
\hline \textbf{Ecosystem}  & {Week 13}  &{Week 14} &{Week 15} &{Week 16}\\\hline
  Western Press &city forces mariupol kyiv killed & city kyiv mariupol civilians lviv &bucha civilians bodies city troops & forces kyiv city military mariupol \\ \hline
 Russia & operation biological forces kiev people &  forces people special operation kiev &bucha,maxar,bodies,satellite,information,media,body & special,donbass,people,donetsk,mariupol,ministry
        \\ \hline
  Chinese &security,countries,peace,conflict,international,situation & president,china,peace,talks,crisis,foreign,wang  &china,countries,crisis,russian,security,peace\ & nato,crisis,russian,security,peace,world \\ \hline
\end{tabular}
\caption{\label{tab:precision} Evaluation of our methodology on 20 different topics (the top 10 topics and 10 random topics). }  
\vspace{-10pt}
\end{table*}




In order to assess how much images shared from the Russian state government appeared on Chinese websites, we again run this analysis, except with images from Russian government accounts on Twitter to see how often they were reposted on Chinese websites indexed by Google.  We find 77 imges that were shared by Russian government officials or media on Twitter that appear on Chinese run websites. 35 of these images were annotated by Google Vision as concerning Ukraine. t


Overall, we see fairly low inter-ecoystem image shar


Lastly, in order to get a sense of the discourse that occurred 

\begin{table}
\centering
\tiny
\begin{tabular}{l|r|l|r}
\multicolumn{2}{c|}{Weibo} & \multicolumn{2}{c}{Twitter} \\\hline
 Domain & {Sourced} &Domain & {Sourced}\\ \hline

Tass & 54 & sputniknews.com & 15 \\\hline 
Sputnik News & 43 & rt.com & 13 \\ \hline
Russia Today  & 82 & ria.ru & 9 \\ \hline
RIA Novosti &58& tass.com  &7\\ \hline

\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting} The total number of posts to each different Russian news source. }  
\vspace{-15pt}
\end{table}
we analyze the resharing and reposting of images about Ukraine from the Russian state media and government on Weibo and by the Chinese government on Twitter. We do so to illustrate directly the extent how Russian framing around the Russo Ukrainian War has permeated different ecosystem.

\paragraph{Direct reposting by Chinese Government Officials and Chinese State Media}
It has been widely reported that the Chinese state media have been helping to spread Russian state disinformation~\cite{Yuan2022, Bandurski2022}, and we see that reflected in the amount of citations given to Russian news stations both on Twitter and on Weibo. Taking our list of 144 Chinese state media accounts from Twitter, gather each tweet in 2022 that mentioned Tass, RT, Sputnik News, or RIA Novosti, as a source for a given story. As see in Table X

\begin{table}
\centering
\tiny
\begin{tabular}{l|r|l|r}
\multicolumn{2}{c|}{Weibo} & \multicolumn{2}{c}{Twitter} \\\hline
 Domain & {Sourced} &Domain & {Sourced}\\ \hline

Tass & 54 & sputniknews.com & 15 \\\hline 
Sputnik News & 43 & rt.com & 13 \\ \hline
Russia Today  & 82 & ria.ru & 9 \\ \hline
RIA Novosti &58& tass.com  &7\\ \hline

\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting} The number of posts that utilize Russian News as sources. }  
\vspace{-15pt}
\end{table}


\begin{table}
\centering
\tiny
\begin{tabular}{l|r|l|r}
\multicolumn{2}{c|}{Twitter} & \multicolumn{2}{c}{Weibo} \\\hline
 Domain & {Number of Photos} &Domain & {Number of Photos}\\ \hline

rt.com & 5 & sputniknews.com & 15 \\\hline 
pikabu.ru &3 & rt.com & 13 \\ \hline
tass.com & 3 & ria.ru & 9 \\ \hline
 sputniknews.com &2 & tass.com  &7\\ \hline
chernayakobra.ru & 2 & nogomi.ru &5 \\ \hline

\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting} The number of photos from each domain that were posted by Chinese state media on Twitter and Weibo. }  
\vspace{-15pt}
\end{table}

\begin{table}
\centering
\tiny
\begin{tabular}{l|r|l|r}
\multicolumn{2}{c|}{Twitter} & \multicolumn{2}{c}{Weibo} \\\hline
\hline  Entity & {Number of Photos}\\ \hline
            China & 564  & Russia & 1870\\\hline 
            Ukraine &397  & China & 1366\\ \hline
            Russia & 344 & Tencent  &1250\\ \hline
            Coronavirus disease 2019 & 160 & Olympic Games Beijing 2022 & 839\\ \hline
            United States& 156 & Ukraine  & 830\\ \hline
            Economy 2022 & 105 & Coronavirus disease 2019  &550\\

\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting} Top entities of Russian images that were shared by Chinese government officials.}  
\vspace{-15pt}
\end{table}


\begin{table}
\centering
\tiny
\begin{tabular}{l|r}
\hline  Entity & {Number of Photos}\\ \hline
Ukraine & 6015 \\\hline 
Russia &4027 \\ \hline
China & 1182 \\ \hline
United States &918 \\ \hline
2022 Russian invasion of Ukraine  & 916\\ \hline
Volodymyr Zelensky & 554 \\ \hline
President of Russia  & 504 \\\hline
Prime minister & 460 \\ \hline
United Kingdom &  440 \\ \hline
European Union & 421 \\ \hline
Russian& 328 \\ \hline
Ukrainians& 314\\ \hline
France & 284\\ \hline
Russo-Ukrainian War & 274\\ \hline
President of the United States & 259\\ \hline
Turkey & 219\\ \hline
Poland & 209 \\ \hline
Germany & 191 \\\hline
Invasion & 177 \\\hline
prelude to the 2022 Russian invasion of Ukraine& 167 \\\hline
NATO& 153 \\\hline
Iran & 131\\\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting} Top entities of about Ukraine by Weibo Ukraine posters.}  
\vspace{-15pt}
\end{table}




, on Twitter, we do not see heavy reposting of images that were also posted on Russian state images.  As seen in Table~\ref{tab:chinese-gov-reposting}, within our timeframe of 2022 only 23 different images were reposted by Chinese state media.  We note that most of these images were fairly innocuous and were just headline picture. We again note the prevalence of images regarding biological weapons in Ukraine that were mutually shared between Chinese and Russian government entities. Of the 90 images from shared from Chinese state media accounts that were also shared by Russian entities, 27 were Ukraine related, one going deep into depth about Hunter Biden's relationship with Ukraine.

While, we saw a lack of evidence of significant reposting of Russian state originated images by Chinese state media, looking at the top posters of Ukrainian related content on Weibo, we see very different behaviour. We do not perform this same analysis for Twitter because since 2009, Twitter has been banned in China~\cite{sullivan2012tale}.

Using the list of the 194 top accounts that posted about Ukraine created by Fung et~\cite{fung2022weibo}, we seek to understand the degree to which these users sourced their images from Russian backed places on the Internet. 

\begin{table}
\centering
\tiny
\begin{tabular}{l|r|}
\multicolumn{2}{c|}{Twitter}  \\\hline
 Domain & {Number of Photos} \\ \hline

ria.ru & 192\\\hline 
sputniknews.com &141  \\ \hline
topwar.ru & 139 \\ \hline
rt.com &116 \\ \hline
9111.ru & 113 \\ \hline
kp.ru & 81 \\ \hline
lenta.ru & 78 \\ \hline
rg.ru & 72 \\ \hline
tass.com &  67 \\ \hline
life.ru & 52 \\ \hline

\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting} The number of photos from each domain that were posted by the most avid Ukraine posters on Wiebo. }  
\vspace{-15pt}
\end{table}

\begin{CJK*}{UTF8}{bsmi}

\begin{table}
\centering
\tiny
\begin{tabular}{l|r|l|r}
\multicolumn{2}{c|}{Weibo}  &\multicolumn{2}{c|}{Twitter} \\\hline
 Word & {NPMI} &  Word & {NPMI}  \\ \hline

尊重/respect		 & 0.225940 &labs & 0.321904	 \\ \hline
天然氣/natural gas		 &0.221828	 & biolabs & 0.345456	 \\ \hline
和解/understanding		 & 0.213163	& kherson & 0.298017	 \\ \hline
歐洲/ Europe		 &0.208866& research & 0.292522 \\ \hline
理由/ reason	 & 0.208032	 &russophobia	 & 0.288264 \\ \hline
俄羅斯人/Russian	 & 0.195902	 &neo-nazis	 & 0.281808 \\ \hline
\hline
\end{tabular}
\caption{\label{tab:chinese-gov-reposting}Words characteristic of the top 20\% of Russian media posts on Twitter and Weibo }  
\vspace{-15pt}
\end{table}
\end{CJK*}



Of the 37,054 pictures, posted 4.46\% were Ukraine related. Of those pictures 13.1\% came from Russian sources 



\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/}
\label{fig:rt}
\end{subfigure}%
\hspace{2pt}

\caption{Examples of image that was shared by Chinese state media on Weibo and reposted by Russian entities. 
}
\label{fig:china-russia-shared-gov-picture}
\vspace{-10pt}
\end{figure}


 More recently, Brennan et al~\cite{brennen2021beyond}, took this same approach to understanding the use of memes and images in the spread of COVID-19 misinformation. Garimella and Eckles~\cite{garimella2020images} found extensive use of images and memes to spread misinformation about elections in Indian Whatsapp groups.  Zannettou et al. found that 90.3\% of the state sponsored accounts in their dataset utilized images/memes~\cite{zannettou2018origins}.  These case studies, among many others, illustrated the widespread use of misleading and altered images for the spread of misinformation.  
 
 
 
 
 
 

Lastly, we quantify the degree to which Russian news sources have influenced the coverage of different Chinese news outlets coverage of Russo-Ukrainian war. We quantify the Russian influence on a given news outlet based on  1) the number of times the news outlet utilized a Russian news outlet as a news source for an article, 2) the number of times the news outlet utilized a photo from a Russian source, and 3) how often the news outlet reuses a hashtag from a Russian account on Weibo. Beginning in February, we observe a large spike in the amounts of citations of Russian news outlets, use of Russian-sourced photos, and Russian-backed hashtags. Posts from Chinese news outlets, that utilized Russian based source received over 4,753,011 reactions on Weibo and nearly 2,287,298 likes on Twitter.  We further find that among the top posters of Ukrainian based content on Weibo  that 11.86\% of the images posted were came from Russian sources.



\begin{figure}
  \centering
\begin{subfigure}{.35\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{LaTeX/figures/chinese-gov-repost0-weibo.jpg}
\label{fig:rt}
\end{subfigure}%
\caption{Examples of an image reposted by CCTV, CGTN, and Global Times that came from a Russian source. The image in question discusses Hunter Biden's (US President Joe Biden's son) connection to Ukraine.
}
\label{fig:china-russia-shared-gov-picture-instance}
\vspace{-10pt}
\end{figure}

==> conclusion.tex <==
\section{Conclusion}

